A Conceptual Introduction to Markov Chain Monte Carlo Methods

Markov Chain Monte Carlo (MCMC) methods have become a cornerstone of many modern scientific analyses by providing a straightforward approach to numerically estimate uncertainties in the parameters of a model using a sequence of random samples. This article provides a basic introduction to MCMC methods by establishing a strong conceptual understanding of what problems MCMC methods are trying to solve, why we want to use them, and how they work in theory and in practice. To develop these concepts, I outline the foundations of Bayesian inference, discuss how posterior distributions are used in practice, explore basic approaches to estimate posterior-based quantities, and derive their link to Monte Carlo sampling and MCMC. Using a simple toy problem, I then demonstrate how these concepts can be used to understand the benefits and drawbacks of various MCMC approaches. Exercises designed to highlight various concepts are also included throughout the article.

==> old <==
\section{Bayesian Inference} \label{sec:bayes}

In many scientific applications, we have access to some \textbf{data} $\data$
that we want to use to make inferences about the world around us.
Most often, we want to interpret these data in light of an underlying
\textbf{model} $M$ that can make predictions about the data we expect
to see as a function of some \textbf{parameters} $\params_M$ of that
particular model.

We can combine both of these pieces together to estimate the
\textbf{probability} $P(\data|\params_M, M)$ 
that we would actually see that data $\data$ we have
collected \textit{conditioned on} (i.e. assuming)
a specific choice of parameters $\params_M$ from our model $M$.
In other words, assuming our model $M$ is right and
the parameters $\params_M$ describes the data, what is the
\textbf{likelihood} $P(\data|\params_M, M)$ that we
actually would observe $\data$? Assuming different values
of $\params_M$ will gives different likelihoods, telling us
which parameter choices appear to best describe the data we
observe.

In Bayesian inference, we are interested in
inferring the opposite quantity $P(\params_M|\data, M)$.
This describes the probability that the 
underlying \textit{parameters} are actually $\params_M$ 
given our data $\data$ and assuming a particular model $M$.
By using factoring of probability, we can relate this new
probability $P(\params_M|\data, M)$ to the likelihood
$P(\data|\params_M, M)$ described above as
\begin{equation}
    P(\params_M | \data, M) P(\data | M) 
    = P(\params_M, \data | M)
    = P(\data | \params_M, M) P(\params_M | M)
\end{equation}
where $P(\params_M, \data | M)$ represents the \textit{joint}
probability of having an underlying set of parameters $\params_M$
that describe the data and observing the particular set of data $\data$
we have already collected.

Rearranging this equality into a more convenient form 
gives us \textbf{Bayes Theorem}:
\begin{equation}
    P(\params_M | \data, M) 
    = \frac{P(\data | \params_M, M) P(\params_M | M)}{P(\data | M)}
\end{equation}
This equation now describes exactly how our two probabilities relate to each other.

As before, $P(\data | \params_M, M)$ is the \textbf{likelihood}. This
describes is the probability that we would have observed our data $\data$
given the parameters $\params_M$ for our particular model $M$. To put this
another way, the likelihood essentially poses the following thought experiment:
if we decide that $\params_M$ is the true underlying parameter values for our
model $M$, what is the probability that we would observe our data $\data$?

$P(\params_M | M)$ is often referred to as the \textbf{prior}. This describes
the probability of having a particular parameter $\params_M$
for our given model $M$ \textit{before conditioning on our data}. In other words:
before we saw our data $\data$, what would be have thought it the probability
that $\params_M$ is actually the true underlying parameter values?
Because this is independent of the data, this term
is often interpreted as representing 
our ``prior beliefs'' about what $\params_M$ \textit{should}
be based on previous measurements, physical concerns, 
and other known factors. In practice, this has the effect of essentially
``augmenting'' the data with other information.

The denominator
\begin{equation}
    P(\data | M) = \int P(\data | \params_M, M) P(\params_M | M) \deriv \params_M
\end{equation}
is known as the \textbf{evidence} or \textbf{marginal likelihood}
for our model $M$ \textit{marginalized} over all possible parameters $\params_M$.
This is a constant that broadly tries to answer the question:
how well does our model $M$ explain the data, averaged over
all possible values $\params_M$ of the true underlying parameters?
Models that do a reasonable job overall thus tend to be favored 
over models that can do a better job sometimes but 
don't perform as well as in general.

Finally, $P(\params_M | \data, M)$ represents our \textbf{posterior}.
This quantifies our belief in $\params_M$ after combining our
prior intuition $P(\params_M|M)$ with
current observations $P(\data|\params_M,M)$ 
and normalizing by the overall evidence $P(\data|M)$.
In other words: given what we knew beforehand and what the data
tells us, what do we think we now know about $\params_M$?
This will always be some compromise between the prior and 
the likelihood, with the exact combination depending
on the strength and properties of the prior and the quality
of the data used to derive the likelihood.

Throughout the rest of the paper we will write 
these four terms (likelihood, prior, evidence, posterior)
using shorthand notation such that
\begin{equation}
    \posterior(\params) 
    \equiv \frac{\likelihood(\params)\prior(\params)}{
    \int \likelihood(\params)\prior(\params) \deriv \params}
    \equiv \frac{\likelihood(\params)\prior(\params)}{\evidence}
    \propto \likelihood(\params)\prior(\params)
\end{equation}
where $\posterior(\params) \equiv P(\params_M | \data, M)$ is the posterior,
$\likelihood(\params) \equiv P(\data | \params_M, M)$ is the likelihood,
$\prior(\params) \equiv P(\params_M | M)$ is the prior, and the constant
$\evidence \equiv P(\data | M)$ is the evidence. We have suppressed the
model subscript for convenience here since in most cases we will only
be examining a single model, but will re-introduce it as necessary.

\subsection{Example: Coin Flips}

As an illustrative example just to explore the basic concepts of
Bayesian inference, let's imagine that we have observations of three
coin flips $\data = \{ H, H, H\}$ from a coin containing a ``heads''
side $H$ and ``tails'' sides $T$.
We would like to infer the probability $p$ that the coin will
come up heads. Assuming all the coin flips are independent, the probability
that all three come up heads is just the product of
the probability of coming up heads each time:
\begin{equation}
    P(\{ H, H, H\} | p) 
    = P(H|p) \times P(H|p) \times P(H|p)
    = p^3
\end{equation}

Using our likelihood, let's now examine two possibilities.
In the first case, let's assume the coin is fair with $p=0.5$
so that we have an equal probability of getting heads or tails.
In this case, the likelihood is
\begin{equation}
    \likelihood_{3H}(p=0.5) = (0.5)^3 = 0.125
\end{equation}

In the second case, let's assume instead that the
coin is totally biased with $p=1$ so that we
always will get heads. We might expect this
behavior if we have a double-sided coin with two
heads. Here, we instead get a likelihood of
\begin{equation}
    \likelihood_{3H}(p=1) = (1)^3 = 1
\end{equation}

Our results imply that, based on the data alone,
the $p=1$ case is 8x more likely than $p=0.5$.
So naively it appears quite likely that
the coin is totally biased.

Our experiences with coins, however, heavily discounts this
view. We intuitively know that seeing three heads in a 
row can occur reasonably often (12.5\% of the time) for 
coins that are fair, and so this probably should not be enough evidence to
believe a coin is biased (let alone by such a substantial amount).

As a starting point, we can probably say
the vast majority of coins we have encountered
have most likely been roughly fair, with $p \approx 0.5$.
That said, we likely haven't experimented with all
of them to confirm this is the case.

Let's try to quantify this intuition. Our
prior should favor the idea that a random coin is fair,
but allow for some uncertainty since we don't know
exactly how much variation there can be between random coins.
As a starting point, let's consider
a truncated Normal distribution centered at $\mu_p=0.5$ with a 
width of $\sigma_p=0.2$:
\begin{equation}
    \prior(p) \approx 2.02 \times
    \begin{cases}
    \exp\left[-\frac{1}{2}\frac{(p - 0.5)^2}{(0.2)^2}\right] & 0 \leq p \leq 1 \\
    0 & {\rm otherwise}
    \end{cases}
\end{equation}
The truncation at $p < 0$ and $p > 1$ codifies the fact that
the chance of getting heads is between 0\% and 100\% (so we can't
have guesses outside of that range). The prior is maximized at
$p=0.5$, giving the most weight to the coin being fair. And
our choice of $\sigma_p=0.2$ means that we believe there is a
roughly 70\% chance that the true value of $p$ lies between
$0.3$ and $0.7$ and a 95\% chance that is between
$0.1$ and $0.9$. And the $0.49$ value just ensures that
our prior integrates to 1.

Given this prior, our posterior for the coin being fair is then
\begin{equation}
    \posterior_{3H}(p=0.5) \approx (2.02) (1) (0.5)^3 \approx 0.25
\end{equation}
while our posterior for it being totally biased is
\begin{equation}
    \posterior_{3H}(p=1) \approx (2.02) (0.04) (1)^3 \approx 0.04
\end{equation}
Compared with our likelihood, our posterior actually points
us to almost the exact opposite answer, informing us that
$p=1$ is roughly 3x \textit{less} probable than $p=0.5$ 
under our prior assumptions. So even though the data haven't changed, 
the inferences based on our observations are completely different.

To get a sense of how our prior belief in fairness impacts these
results, let's consider the case where we could observe some more coin flips.
How many consecutive heads would it take to prefer 
$p=1$ over $p=0.5$? It turns out it takes no fewer than 
$n=5$ consecutive heads to get an posterior probability
\begin{equation}
    \posterior_{5H}(p=0.5)
    \approx (2.02) (1) (0.5)^5
    \approx 0.06 < 0.08
\end{equation}
that even slightly disfavors $p=0.5$. Put another way, 
our prior belief that the coin is somewhat fair means 
we would need to observe at least five heads in a row
before we might start to favor the explanation that
something suspicious might be going on (i.e. $p=1$).

This example highlights one extremely crucial element to
any Bayesian analysis: \textit{the interpretation of any result is
only as good as the models and priors that underlie them}.
Trying to explore the implications of any particular model
is fundamentally a secondary concern behind constructing 
a reasonable model with well-motivated priors. 
We strongly encourage readers to keep this idea in mind
throughout the remainder of this work.

\section{What are Posteriors For?} \label{sec:what}

Above, we described how Bayes Theorem is able to combine
our prior beliefs and the observed data into a new posterior estimate 
$\posterior(\params) \propto \likelihood(\params) \prior(\params)$.
We also showed how this can work in practice using a simple example
involving coin flips to highlight how different prior beliefs
can impact our interpretation of the data.

This, however, is only half of the problem. Once we have
the posterior, we need to then \textit{use} it to
make inferences about the world around us. For instance,
in the coin-flipping example we explored above, we examined how much
the posterior favored one particular value for the probability $p$
of landing on heads versus another.

In general, the ways in which we want to use posteriors
fall into four broad categories:
\begin{enumerate}
    \item \textbf{Making educated guesses}:
    make a reasonable guess at what the underlying model parameters are.
    \item \textbf{Quantifying uncertainty}:
    provide constraints on the range of possible parameter values.
    \item \textbf{Generating predictions}:
    marginalize over uncertainties in the underlying parameters 
    to predict what will happen next.
    \item \textbf{Comparing models}:
    use the evidences from different models
    to try and favor some models over others.
\end{enumerate}

In order to do accomplish these goals,
we are often more interested in trying to use the
posterior to estimate various constraints on the parameters
$\params$ themselves or other quantities $f(\params)$ that
might be based on them. For instance, in the coin-flipping
example above, we might try to ask questions such as:
\begin{itemize}
    \item What is our best guess for $p$?
    \item What values of $p$ can we rule out?
    \item What are the chances the next three coin flips
    will be heads?
    \item Is our original model well-motivated compared
    with possible alternatives?
\end{itemize}

In general, questions like these depend on marginalizing
(i.e. \textit{integrating}) over the uncertainties 
characterized by our posterior (via the likelihood
and prior). The evidence, for instance, is again just the integral
of the likelihood and the prior over all possible parameters:
\begin{equation}
    \evidence 
    = \int \likelihood(\params) \prior(\params) \deriv \params
\end{equation}
Likewise, if we are interested in just the behavior of a subset of
parameters $\params_{\rm int}$ from 
$\params = \{ \params_{\rm int}, \params_{\rm nuis} \}$,
we can marginalize over the behavior of the 
``nuisance'' parameters $\params_{\rm nuis}$ to get:
\begin{equation}
    \posterior(\params_{\rm int}) 
    = \int \posterior(\params) \deriv \params_{\rm nuis}
    = \int \posterior(\params_{\rm int}, \params_{\rm nuis}) \, \deriv \params_{\rm nuis}
\end{equation}

Other quantities can generally be derived from the \textbf{expectation value}
of various parameter-dependent functions $f(\params)$ with respect to the posterior:
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \equiv \frac{\int f(\params) \posterior(\params) \deriv \params}
    {\int \posterior(\params) \deriv \params} 
    = \frac{\int f(\params) \likelihood(\params) \prior(\params) \deriv \params}
    {\int \likelihood(\params) \prior(\params) \deriv \params}
\end{equation}
This represents a weighted average of $f(\params)$
where at each value $\params$ we weight the resulting
$f(\params)$ proportional to the chance we believe that value is correct 
$\posterior(\params) \propto \likelihood(\params) \prior(\params)$.

Taken together, we see that \textit{in almost all cases we are usually
more interested in computing integrals over the posterior
rather than knowing the posterior itself.}
Asking even basic questions like ``Is my coin fair?''
not only requires computing the posterior for a specific value ($p=0.5$) but 
likely comparing it to all other possible values ($p \neq 0.5$).
To put this another way, the posterior is rarely ever useful on its
own; it becomes useful by integrating over it.

This distinction between estimating expectations
$\meanwrt{f(\params)}{\posterior}$ and other integrals
over the posterior versus estimating the posterior 
$\posterior(\params)$ in-and-of-itself is a key element of Bayesian inference.
This distinction is hugely important when it comes
to actually doing inference in practice, since it
is often the case that we can get an excellent estimate of
$\meanwrt{f(\params)}{\posterior}$ even if we have an
extremely poor estimate of $\posterior(\params)$.

\subsection{Making Educated Guesses} \label{subsec:guess}

One of the core tenets of Bayesian inference is that
we don't know the true model $M_*$ or its underlying parameters
$\params_*$ that characterize the data we observe. If
we assume that our current model $M$ is correct, however,
we can try to use our posterior $\posterior(\params)$
to propose a \textbf{point estimate} $\hat{\params}$
that we think is a pretty good guess for $\params_*$.

What exactly counts as ``good''? This depends on exactly what we care
about. In general, we can quantify this by asking the opposite question:
how badly are we penalized if our estimate $\hat{\params} \neq \params_*$
is wrong? This is often encapsulated through the use of
a \textbf{loss function} $L(\hat{\params}|\params_*)$
that penalizes us when our point estimate $\hat{\params}$
is not equal to $\params_*$. Common loss functions 
include \textbf{squared loss}
\begin{equation}
    L(\hat{\params}|\params_*) = |\hat{\params} - \params_*|^2
\end{equation}
where the penalty goes as the square of the magnitude of the offset,
\textbf{absolute loss}
\begin{equation}
    L(\hat{\params}|\params_*) = |\hat{\params} - \params_*|
\end{equation}
where the penalty is directly proportional to the magnitude of the offset,
and \textbf{0-1 loss}
\begin{equation}
    L(\hat{\params}|\params_*) = \indicator{|\hat{\params} - \params_*| \neq 0}
\end{equation}
where
\begin{equation}
    \indicator{|\hat{\params} - \params| \neq 0}
    = \begin{cases}
    1 & |\hat{\params} - \params| \neq 0 \\
    0 & {\rm otherwise}
    \end{cases}
\end{equation}
is the \textbf{indicator function} which evaluates to $1$
if the condition is true and $0$ otherwise. In other words,
0-1 loss gives a flat penalty for any point estimate $\hat{\params}$
that doesn't agree \textit{exactly} with the underlying
$\params_*$ (and no penalty if it does).

Unfortunately, we don't know what the actual value of
$\params_*$ is to actually evaluate the loss. However,
we can do the next best thing and compute the \textbf{expected loss}
averaged over all possible values of $\params_*$ based on
our posterior:
\begin{equation}
    L_\posterior(\hat{\params})
    \equiv \meanwrt{L(\hat{\params}|\params)}{\posterior}
\end{equation}
The best guess we can make then is to choose our point estimate
$\hat{\params}$ to be one that minimizes the expected loss
\begin{equation}
    \hat{\params} 
    \equiv \argmin_{\params} \left[L_\posterior(\params)\right]
\end{equation}
So we see that trying to do something as simple as just making
a good guess requires integrating over the posterior.

While this strategy can work for any arbitrary loss function, solving
for $\hat{\params}$ often requires using numerical methods and repeated
integration over $\posterior(\params)$.
However, for the three specific loss functions 
we explored above, it can be shown that the optimal point estimate
$\hat{\params}$ ends up being:
\begin{itemize}
    \item the \textbf{mean} of the posterior under squared loss,
    \item the \textbf{median}\footnote{
    Note that since the median is not uniquely defined in more than one
    dimension, absolute loss ultimately gives rise to an
    entire \textit{class} of optimal estimates in higher dimensions.}
    of the posterior under absolute loss, and
    \item the \textbf{mode} of the posterior under 0-1 loss.
\end{itemize}

As an illustration of how this works in practice,
let's return to our coin flipping example. Our posterior
$\posterior_{3H}(p)$ for $p$ after three heads is
\begin{equation}
    \posterior_{3H}(p) \approx
    11.24 \times
    \begin{cases}
    p^3 \exp\left[-\frac{1}{2}\frac{(p - 0.5)^2}{(0.2)^2}\right] & 0 \leq p \leq 1 \\
    0 & {\rm otherwise}
    \end{cases}
\end{equation}
where the normalizing factor of $11.24 \approx \evidence^{-1}$
again just ensures the posterior integrates to 1.

Solving for $p_{\rm mean}$ gives
\begin{equation}
    \hat{p}_{\rm mean} 
    \equiv \meanwrt{p}{\posterior}
    = \int p \, \posterior_{3H}(p) \deriv p
    \approx 0.672
\end{equation}
Solving for $p_{\rm med}$ gives
\begin{equation}
    \int_0^{\hat{p}_{\rm med}} \posterior_{3H}(p) \deriv p
    = \int_{\hat{p}_{\rm med}}^1 \posterior_{3H}(p) \deriv p
    \quad \Rightarrow \quad \hat{p}_{\rm med} \approx 0.676
\end{equation}
Solving for $p_{\rm mode}$ gives
\begin{equation}
    \hat{p}_{\rm mode} 
    \equiv \argmax_{p} \left[\posterior_{3H}(p)\right]
    \approx 0.677
\end{equation}
Finally, let's consider an alternate, more ``conservative'' loss function
\begin{equation}
    L_{\rm cons}(\hat{p}|p_*) = |\hat{p} - p_*|^5
\end{equation}
that penalizes us much more heavily for guessing 
values that are further away from the true $p_*$. This gives:
\begin{equation}
    \hat{p}_{\rm cons} = \argmin_{\hat{p}}
    \left[\int_0^1 |\hat{p} - p |^5 \posterior_{3H}(p) \deriv p \right]
    \approx 0.657
\end{equation}

We first notice that all our estimates are prefer values of $p > 0.5$.
This occurs because the likelihood $\likelihood_{3H}(p) \propto p^3$
prefers larger values of $p$ given the observed string of heads
even though our prior $\prior(p)$ is symmetric around $p=0.5$.
This showcases the impact the data (three consecutive heads) has
on our point estimate.

In addition, we see all our estimates give slightly different answers,
with the estimate $\hat{p}$ decreasing as our loss function becomes
more strict, with $\hat{p}_{\rm mode} \approx 0.677$ with 0-1 loss,
$\hat{p}_{\rm med} \approx 0.676$ with absolute loss, 
$\hat{p}_{\rm mean} \approx 0.672$ with squared loss,
and $\hat{p}_{\rm cons} \approx 0.657$ with more conservative
quintic loss. This occurs because of the asymmetry in our posterior:
although our posterior implies that there is a greater chance that
$p_* > 0.5$, there is a non-zero chance that it could be smaller.
If that is the case, we would be further off than if we had guessed
a smaller number, leading to a proportionately larger penalty
and consequently estimates closer to $p=0.5$. In other words,
the larger our penalty for $\hat{p}$ being far away from $p_*$,
the more we try and guard against the worst possible case
instead of looking for the best possible case.

\subsection{Quantifying Uncertainty} \label{subsec: guess}

In many cases, we are not just interested in computing
a prediction $\hat{\params}$ for $\params_*$ but also constraining
a region $\credible(\params)$ of possible values 
that $\params_*$ might be with some amount of certainty.
In other words, can we construct a region $\credible_X$
such that we believe there is an $X\%$ chance that it contains
$\params_*$?

There are infinitely many possible definitions
for this \textbf{credible region}. One unique definition,
however, is defining it to be
the region(s) above some posterior threshold $\posterior_X$
where $X\%$ of the posterior is contained, i.e. where
\begin{equation}
    \int_{\params \,\in\, \credible_X} \posterior(\params) \deriv \params
    = X/100
\end{equation}
given
\begin{equation}
    \credible_X
    \equiv \left\{ \params : \posterior(\params) \geq \posterior_X \right\}
\end{equation}
\textbf{An example of how this works is shown in schematic figure}.

Returning to our coin-flipping example, let's try to compute
the 1-D \textbf{credible interval} defined above 
for various levels of credibility. If we want to define the 70\%
credible interval for $p$, we find that
\begin{equation}
    \posterior_{70} \approx 1.47
    \quad \Rightarrow \quad
    \credible_{70} \approx [0.508, 0.853]
\end{equation}
where $[0.508, 0.853]$ encompasses all values of $p$ from $p=0.508$
to $p=0.853$, inclusive.
Likewise, the 95\% credible interval is
\begin{equation}
    \posterior_{95} \approx 0.57
    \quad \Rightarrow \quad
    \credible_{95} \approx [0.389, 0.985]
\end{equation}
So we are 70\% certain that the true $p_*$ is within
$[0.508,0.853]$ and 95\% certain that it lies between
$[0.389, 0.985]$. This allows us to try and rule out values
of $p_*$ being outside of these regions provided we are
comfortable with having a 100-X\% chance of being wrong.
For instance, there is only a 5\% chance
that $p < 0.389$ or $p > 0.985$, so we might feel relatively
confident saying that $p \neq 1$ given the data we have.

\subsection{Making Predictions} \label{subsec:pred}

In addition to trying to estimate the underlying parameters of our
model, we often also want to make predictions about what might happen next.
If we think we know the underlying true model parameters $\params_*$
this process is straightforward. We, however, only have access to the
posterior distribution $\posterior(\params)$ over possible
values $\params_*$ could take. Predicting what will happen thus
requires marginalizing over this uncertainty.

We can quantify this intuition using the \textbf{posterior predictive}:
\begin{equation}
    P(\tilde{\data}|\data) 
    \equiv \int P(\tilde{\data}|\params) P(\params|\data) \deriv \params
    \equiv \int \tilde{\likelihood}(\params) \posterior(\params) \deriv \params
    = \meanwrt{\tilde{\likelihood}(\params)}{\posterior}
\end{equation}
This represents the likelihood $\tilde{\likelihood}(\params)$
of seeing hypothetical data $\tilde{\data}$ after averaging over all possible
values of $\params$ based on the current posterior $\posterior(\params)$.

Let's return to our coin-flipping example to again get a sense of 
how the posterior predictive works in practice. Say we are interested
in the probability that the \textit{next} three coin tosses will
also be heads. The probability of that occurring is
\begin{equation}
    \tilde{\likelihood}(p) = \likelihood_{3H}(p) = p^3
\end{equation}
Plugging this into our expression for the posterior predictive gives
\begin{equation}
    P({\rm 3\:more\:heads} \,|\, {\rm 3\:heads})
    = \int_0^1 p^3 \posterior_{3H}(p) \deriv p
    \approx 0.35
\end{equation}

What does this tell us? Naively, if we expected our coin was fair,
the chance of getting three more heads would just be $(0.5)^3=0.125$
(12.5\%). However, after witnessing a previous string of heads,
our posterior belief is that the coin is more likely to be biased
with $p>0.5$. This gives a higher likelihood of getting a subsequent
string of heads, with the likelihood favoring larger biases
since it goes as $\propto p^3$.

As a sanity check, we can also compute the posterior predictive
for the other three options: two heads and one tail, two tails and
one heads, and three tails. Including contributions from random
permutations (i.e. $\{ H, H, T\}$, $\{ H, T, H\}$, and $\{ T, H, H\}$
all are two heads and one tail, etc.), we get:
\begin{align}
    P({\rm 2\:more\:heads,\:1\:tails} \,|\, {\rm 3\:heads})
    &= \int_0^1 3 p^2 (1-p) \posterior_{3H}(p) \deriv p
    \approx 0.37 \\
    P({\rm 1\:more\:heads,\:2\:tails} \,|\, {\rm 3\:heads})
    &= \int_0^1 3 p (1-p)^2 \posterior_{3H}(p) \deriv p
    \approx 0.22 \\
    P({\rm 3\:tails} \,|\, {\rm 3\:heads})
    &= \int_0^1 (1-p)^3 \posterior_{3H}(p) \deriv p
    \approx 0.06
\end{align}
The combined sum of all possible outcomes is
$0.35 + 0.37 + 0.22 + 0.06 = 1$, as expected.

\subsection{Comparing Models} \label{subsec:evid}

One final point of interest in many Bayesian analyses is
trying to investigate whether the data particularly favor
any of the model(s) we are assuming in our analysis.
Our choice of priors or the particular way we parameterize the
data can lead to substantial differences in the way we
might want to interpret our results.

In Bayesian inference, we can compare two models by computing
the \textbf{Bayes factor}:
\begin{equation}
    \bayesfactor
    \equiv \frac{P(M_{\rm 1}|\data)}{P(M_{\rm 2}|\data)}
    = \frac{P(\data|M_{\rm 1})P(M_{\rm 1})}{P(\data|M_{\rm 2})P(M_{\rm 2})}
    = \frac{\evidence_{\rm 1}}{\evidence_{\rm 2}} 
    \frac{\prior_{\rm 1}}{\prior_{\rm 2}}
\end{equation}
where $\evidence_M$ is again the evidence for model $M$ 
and $\prior_M$ is our prior belief that $M$ 
is correct relative to the competing model.
Taken together, the Bayes factor $\bayesfactor$ tells us
how much a particular model is favored over another given the
observed data, marginalizing over all possible values of the underlying
model parameters $\params_M$, and our previous relative confidence in the model.

Again, let's return to our coin-flipping example to get a sense for how this
works. As our starting model we'll consider the prior we've been using in
our previous examples. Plugging in and integrating gives
\begin{equation}
    \evidence_0
    \equiv \int_0^1 \likelihood_{3H}(p) \prior(p|M_0) \deriv p
    \approx 2.02 \int_0^1 p^3 
    \exp\left[-\frac{1}{2}\frac{(p - 0.5)^2}{(0.2)^2}\right] \deriv p
    \approx 0.18
\end{equation}

Let's consider two alternatives. In the first case, we
assume the coin is completely fair so that $p=0.5$. This means
our prior is effectively
\begin{equation}
    \prior(p|M_{\rm fair}) = \delta(p - 0.5)
\end{equation}
where $\delta(p-0.5)$ is the Dirac delta function
centered at $p=0.5$. This gives an evidence of
\begin{equation}
    \evidence_{\rm fair} 
    = \int_0^1 p^3 \delta(p-0.5) \deriv p
    = \left. p^3 \right|_{p=0.5}
    = (0.5)^3 = 0.125
\end{equation}
In the second, we will instead assume there is no reason 
for us to express any preferences for a particular value of $p$.
The prior in that case is just
\begin{equation}
    \prior(p|M_{\rm unif}) = 1
\end{equation}
This gives an evidence of
\begin{equation}
    \evidence_{\rm unif}
    = \int_0^1 p^3 \deriv p
    = 0.25
\end{equation}

Let's assume we're not particularly confident in any model
relative to each other such that 
$\prior_0 = \prior_{\rm fair} = \prior_{\rm unif} = 1/3$.
We see that the largest Bayes factor is between 
$M_{\rm fair}$ and $M_{\rm unif}$, where
\begin{equation}
    \bayesfactor^{\rm unif}_{\rm fair}
    = \frac{\evidence_{\rm unif}}{\evidence_{\rm fair}}
    \frac{\prior_{\rm unif}}{\prior_{\rm fair}}
    = \frac{0.25}{0.125}\frac{1/3}{1/3} 
    = 2
\end{equation}
This indicates that, given the data and our prior
beliefs in which model is right, the data prefer
$M_{\rm unif}$ over $M_{\rm fair}$ (i.e. weaker assumptions)
by a factor of two. As a rule of thumb, we generally want
$\bayesfactor \gg 1$ before being confident that the data
substantially favors one model over the other.

\subsection{Example: Linear Regression}

3-D example that can highlight: corner plots (marginalization),
Gaussian behavior. Better lead in to subsequent section.

\section{Posterior Estimation with Grids}

In many modern analyses involving complicated data and models, the posterior
$\posterior(\params)$ that we are interested in estimating is often significantly
more complicated than the simple examples we looked at above.
It should then be no surprise that many posteriors 
end up being intractable analytically and must be estimating using
numerical methods (as with our previous example).

% \subsection{``Brute Force'' Approach}

% The easiest way to estimate our posterior is to imagine
% that we can estimate it using something like a
% \textbf{Riemann sum} assuming $\params$ is 1-D. Then,
% for a \textbf{grid} of $n$ parameter values 
% $\{ \params_1, \dots, \params_n \}$, the expectation value
% can be approximated by:
% \begin{equation}
%     \meanwrt{f(\params)}{\posterior} 
%     = \frac{\int f(\params) \posterior(\params) \deriv \params}
%     {\int \posterior(\params) \deriv \params}
%     \approx \frac{\sum_{i=1}^{n} f(\params_i) 
%     \posterior(\params_i) \Delta \params_i}
%     {\sum_{i=1}^{n} \posterior(\params_i) \Delta \params_i}
% \end{equation}
% This approximation immediately suggests an associated
% weight
% \begin{equation}
%     w_i = \posterior(\params_i) \Delta \params_i
% \end{equation}
% This result can be immediately generalized
% to higher dimensions, in which case
% \begin{equation}
%     \Delta \params_i = \prod_{j=1}^{d} \Delta \Theta_i^j
% \end{equation}
% is instead the volume of the associated $d$-dimensional
% cuboid with width $\Theta_i^j$ in the $j$th dimension.

% While the exact value of $\posterior(\params_i)$
% is not known beforehand due to the unknown normalizing constant
% $\evidence$, we can easily define our weights instead to be
% \begin{equation}
%     w_i 
%     = \likelihood(\params_i) \prior(\params_i) \Delta \params_i
%     \propto \posterior(\params_i) \Delta \params_i
% \end{equation}
% without changing our expectation value since the additional
% constant cancels out. We can then derive a separate estimate
% of the evidence via
% \begin{equation}
%     \evidence 
%     = \int \likelihood(\params) \prior(\params) \deriv \params
%     \approx \sum_{i=1}^{n} \likelihood(\params_i)
%     \prior(\params_i) \Delta \params_i = \sum_{i=1}^{n} w_i
% \end{equation}

% This procedure gives us a straightforward recipe for
% generating $\hat{\posterior}(\params)$:
% \begin{enumerate}
%     \item Create a $d$-dimensional grid
%     with $n=\prod_{j=1}^d n_j$ total points
%     using $n_j$ points in each dimension.
%     \item Compute the weight 
%     $w_i = \likelihood(\params_i) \prior(\params_i) \Delta \params_i$
%     over each point $\params_i$.
% \end{enumerate}

% While this approach is easy, it has a number of immediate drawbacks.
% The first and most severe is that the total number of samples
% increases \textit{exponentially} as the number of dimensions
% increases:
% \begin{equation}
%     n = \prod_{j=1}^{d} n_j \sim k^d
% \end{equation}
% where $k \geq 2$. This means that even in the absolute
% \textit{best} case we have $2^d$ scaling. This awful scaling
% is often referred to as the \textbf{curse of dimensionality}.

% The second drawback is that the weights can depend sensitively
% on the spacing of the grid. If we do not specify our grid
% well, we might end up with large variations in the derived weights
% since we might spend, e.g., a lot of effort sampling regions where
% $\posterior(\params)$ is small. In the ideal case then, we may
% want to try and increase the resolution of the grid
% in regions where the posterior is large and decrease it elsewhere.

% This suggests that we might be able to come up with
% a better estimator $\hat{\posterior}(\params)$
% (where the weights vary less) using the same number of
% grid points. Conversely, this also implies that we probably
% come up with an estimate that is \textit{at least} as good
% as the one we currently have using a possibly smaller number
% $n_{\rm eff} \leq n$ of grid points. We refer to this
% as the \textbf{effective sample size}.
% Assuming the weights are (re-)normalized such that
% \begin{equation}
%     p_i \equiv \frac{w_i}{n^{-1} \sum_{i=1}^{n} w_i} 
%     \quad\Rightarrow\quad \sum_{i=1}^{n} p_i = n
% \end{equation}
% this is often taken to be (Kish 1965):
% \begin{equation}
%     n_{\rm eff} 
%     \equiv \frac{\left(\sum_{i=1}^{n} p_i\right)^2}{\sum_{i=1}^{n} p_i^2}
% \end{equation}
% We see that in the best case where all the weights are equal ($p_i = 1$)
% this reduces to 
% \begin{equation}
%     n_{\rm eff}^{\rm best}
%     = \frac{\left(\sum_{i=1}^{n} 1\right)^2}{\sum_{i=1}^{n} 1^2}
%     = \frac{n^2}{n} = n
% \end{equation}
% while in the worst case where
% all the weight is concentrated in a single point 
% ($p_i = n$ for $i=j$ and $p_i=0$ otherwise) 
% this reduces to
% \begin{equation}
%     n_{\rm eff}^{\rm worst}
%     = \frac{n^2}{n^2}
%     = 1
% \end{equation}
% In general, errors on estimated quantities scale as a function
% of $n_{\rm eff}$ rather than $n$. For instance, the error on the
% mean is typically goes as $\propto n_{\rm eff}^{-1/2}$.

\section{Estimating the Posterior with Samples}

\textbf{REORGANIZE.}

In many modern analyses involving complicated data and models, the posterior
$\posterior(\params)$ (and evidence $\evidence$) 
that we are interested in estimating is often
intractable analytically and must be estimating using numerical methods.
A particular way of doing this is approximating the posterior density $\posterior(\params)$
using a discrete collection of $n$ \textbf{samples} $\{ \params_1, \dots, \params_n \}$
and associated \textbf{weights} $\{ w_1, \dots, w_n \}$. This can allow us to construct
posterior approximations using methods such as
\textbf{kernel density estimation} (KDE) such that
\begin{equation}
    \posterior(\params) 
    \approx \hat{\posterior}(\params)
    \equiv \frac{n^{-1} \sum_{i=1}^{n} w_i K_i(\params|\params_i)}
    {n^{-1} \sum_{i=1}^{n} w_i}
\end{equation}
where $K_i(\params|\params_i)$ is the \textbf{probability density function (PDF)}
of the \textbf{kernel} associated with sample $\params_i$.
As an example, we can imagine that $K_i(\params|\params_i)$
might be a multivariate Gaussian
\begin{equation}
    K_i(\params|\params_i) 
    = \frac{1}{|2\pi\cov_i|^{1/2}} \exp\left[-\frac{1}{2} 
    (\params - \meanvec_i)^T \cov^{-1} (\params - \meanvec_i) \right]
\end{equation}
with mean $\meanvec_i$ and covariance $\cov_i$, where $T$ is the transpose operator.
The posterior approximation $\hat{\posterior}(\params)$ is then a
\textbf{Gaussian mixture model} with $n$ components.


Without loss of generality, here we will instead consider the simpler approximation:
\begin{equation}
    \posterior(\params) 
    \approx \hat{\posterior}(\params)
    \equiv \frac{n^{-1} \sum_{i=1}^{n} w_i \delta(\params|\params_i)}
    {n^{-1} \sum_{i=1}^{n} w_i}
\end{equation}
where $\delta(\params|\params_i)$ is a Dirac delta function located at
$\params_i$. This particular approximation is appealing because it allows
to easily compute \textbf{expectation values} of other distributions of interest
$f(\params)$ with respect to the posterior:
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \equiv \frac{\int f(\params) \posterior(\params) \deriv \params}
    {\int \posterior(\params) \deriv \params}
    \approx \frac{\int f(\params) \hat{\posterior}(\params) \deriv \params}
    {\int \hat{\posterior}(\params) \deriv \params}
    = \frac{n^{-1} \sum_{i=1}^{n} w_i f(\params_i)}
    {n^{-1} \sum_{i=1}^{n} w_i}
\end{equation}
In other words, we can compute expectation values over arbitrary functions
by just computing the weighted average of the function evaluated over our set of
samples $\{ \params_1, \dots, \params_n \}$ and weights $\{ w_1, \dots, w_n \}$.
This computation is extremely easy to perform and is valid for
any arbitrary function $f(\params)$.

We will deal with the problem of how to pick our
samples $\{ \params_1, \dots, \params_n \}$ and
compute their weights $\{ w_1, \dots, w_n \}$ shortly.
In general though, we can probably expect that this
approximation should be reasonable if:
\begin{enumerate}
    \item Our samples have sufficient \textbf{coverage} so that
    the region(s) of parameter space covered
    by our samples is where the majority (e.g., 99\%) of the
    posterior $\posterior(\params)$ is located.
    \item Our \textbf{effective sample size} is reasonably
    large. This means that either our weights $\{ w_1, \dots, w_n \}$
    don't vary too dramatically or we have a lot
    of samples to make up for it in case they do.
\end{enumerate}

\subsection{``Brute Force'' Approach}

The easiest way to estimate our posterior is to imagine
that we can estimate it using something like a
\textbf{Riemann sum} assuming $\params$ is 1-D. Then,
for a \textbf{grid} of $n$ parameter values 
$\{ \params_1, \dots, \params_n \}$, the expectation value
can be approximated by:
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    = \frac{\int f(\params) \posterior(\params) \deriv \params}
    {\int \posterior(\params) \deriv \params}
    \approx \frac{\sum_{i=1}^{n} f(\params_i) 
    \posterior(\params_i) \Delta \params_i}
    {\sum_{i=1}^{n} \posterior(\params_i) \Delta \params_i}
\end{equation}
This approximation immediately suggests an associated
weight
\begin{equation}
    w_i = \posterior(\params_i) \Delta \params_i
\end{equation}
This result can be immediately generalized
to higher dimensions, in which case
\begin{equation}
    \Delta \params_i = \prod_{j=1}^{d} \Delta \Theta_i^j
\end{equation}
is instead the volume of the associated $d$-dimensional
cuboid with width $\Theta_i^j$ in the $j$th dimension.

While the exact value of $\posterior(\params_i)$
is not known beforehand due to the unknown normalizing constant
$\evidence$, we can easily define our weights instead to be
\begin{equation}
    w_i 
    = \likelihood(\params_i) \prior(\params_i) \Delta \params_i
    \propto \posterior(\params_i) \Delta \params_i
\end{equation}
without changing our expectation value since the additional
constant cancels out. We can then derive a separate estimate
of the evidence via
\begin{equation}
    \evidence 
    = \int \likelihood(\params) \prior(\params) \deriv \params
    \approx \sum_{i=1}^{n} \likelihood(\params_i)
    \prior(\params_i) \Delta \params_i = \sum_{i=1}^{n} w_i
\end{equation}

This procedure gives us a straightforward recipe for
generating $\hat{\posterior}(\params)$:
\begin{enumerate}
    \item Create a $d$-dimensional grid
    with $n=\prod_{j=1}^d n_j$ total points
    using $n_j$ points in each dimension.
    \item Compute the weight 
    $w_i = \likelihood(\params_i) \prior(\params_i) \Delta \params_i$
    over each point $\params_i$.
\end{enumerate}

While this approach is easy, it has a number of immediate drawbacks.
The first and most severe is that the total number of samples
increases \textit{exponentially} as the number of dimensions
increases:
\begin{equation}
    n = \prod_{j=1}^{d} n_j \sim k^d
\end{equation}
where $k \geq 2$. This means that even in the absolute
\textit{best} case we have $2^d$ scaling. This awful scaling
is often referred to as the \textbf{curse of dimensionality}.

The second drawback is that the weights can depend sensitively
on the spacing of the grid. If we do not specify our grid
well, we might end up with large variations in the derived weights
since we might spend, e.g., a lot of effort sampling regions where
$\posterior(\params)$ is small. In the ideal case then, we may
want to try and increase the resolution of the grid
in regions where the posterior is large and decrease it elsewhere.

This suggests that we might be able to come up with
a better estimator $\hat{\posterior}(\params)$
(where the weights vary less) using the same number of
grid points. Conversely, this also implies that we probably
come up with an estimate that is \textit{at least} as good
as the one we currently have using a possibly smaller number
$n_{\rm eff} \leq n$ of grid points. We refer to this
as the \textbf{effective sample size}.
Assuming the weights are (re-)normalized such that
\begin{equation}
    p_i \equiv \frac{w_i}{n^{-1} \sum_{i=1}^{n} w_i} 
    \quad\Rightarrow\quad \sum_{i=1}^{n} p_i = n
\end{equation}
this is often taken to be (Kish 1965):
\begin{equation}
    n_{\rm eff} 
    \equiv \frac{\left(\sum_{i=1}^{n} p_i\right)^2}{\sum_{i=1}^{n} p_i^2}
\end{equation}
We see that in the best case where all the weights are equal ($p_i = 1$)
this reduces to 
\begin{equation}
    n_{\rm eff}^{\rm best}
    = \frac{\left(\sum_{i=1}^{n} 1\right)^2}{\sum_{i=1}^{n} 1^2}
    = \frac{n^2}{n} = n
\end{equation}
while in the worst case where
all the weight is concentrated in a single point 
($p_i = n$ for $i=j$ and $p_i=0$ otherwise) 
this reduces to
\begin{equation}
    n_{\rm eff}^{\rm worst}
    = \frac{n^2}{n^2}
    = 1
\end{equation}
In general, errors on estimated quantities scale as a function
of $n_{\rm eff}$ rather than $n$. For instance, the error on the
mean is typically goes as $\propto n_{\rm eff}^{-1/2}$.

\subsection{Importance Sampling}

Above, we outlined how we can relate a grid of $n$ points to their
associated weights $w_i$ when computing $\hat{\posterior}(\params)$,
how we might change the resolution of the grid to adjust those weights,
and how the distribution of those weights is related to the effective
sample size. Now we want to take this basic idea one step further.

In general, the weight $w_i$ associated with each sample $\params_i$ is
intimately related to the process by which we generated the
entire set of samples. In the case where these are regularly spaced,
$w_i$ is proportional to the value of the posterior at a given position
$\posterior(\params_i)$ as well as the spacing of the grid $\Delta \params_i$.
Decreasing the spacing (making grid denser) decreases the weight since we
now have more points located in that region. This makes sense:
if we roughly double the number of points, each of them should probably
get around half the weight (assuming $\posterior(\params)$ doesn't change
too much).

We can extend this basic relationship between the \textit{density} of points
and their overall weights beyond just changing the resolution of our grid.
Taking this to its conceptual limit, we could imagine estimating
the posterior using an infinite amount of grid points whose spacing/density
changes as a function of $\params$. Let's define the density
as a function of position to be $\proposal(\params)$. 
Using $\proposal(\params)$, we can rewrite our original expectation value
as
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \equiv \frac{\int f(\params) \posterior(\params) \deriv \params}
    {\int \posterior(\params) \deriv \params}
    = \frac{\int f(\params) \frac{\posterior(\params)}{\proposal(\params)}
    \proposal(\params) \deriv \params}
    {\int \frac{\posterior(\params)}{\proposal(\params)}
    \proposal(\params) \deriv \params}
\end{equation}

This may mostly seem like a mathematical trick, but rewriting the result
this way allows us to use the approximation 
\begin{equation}
    \proposal(\params) 
    \approx \hat{\proposal}(\params)
    \equiv \frac{n^{-1} \sum_{i=1}^{n} q_i \delta(\params|\params_i)}
    {n^{-1} \sum_{i=1}^{n} q_i}
\end{equation}
rather than $\hat{\posterior}(\params)$ when trying to compute our results.
Plugging this into our initial expression gives
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \approx \frac{\int f(\params) \frac{\posterior(\params)}{\proposal(\params)}
    \hat{\proposal(\params)} \deriv \params}
    {\int \frac{\posterior(\params)}{\proposal(\params)}
    \hat{\proposal(\params)} \deriv \params}
    = \frac{n^{-1} \sum_{i=1}^{n} f(\params_i)
    \frac{\posterior(\params_i)}{\proposal(\params_i)} q_i}
    {n^{-1} \sum_{i=1}^{n} \frac{\posterior(\params_i)}{\proposal(\params_i)} q_i}
\end{equation}

There are two primary benefits from moving from an adaptively-spaced grid
to a continuous distribution $\proposal(\params)$. First, a grid will
always have some minimum resolution $\Delta \params_i$ that makes it difficult
to get our weights to be \textit{exactly} uniform, limiting our maximum
effective sample size. By contrast, we can in theory get
$\proposal(\params)$ to exactly match the posterior $\posterior(\params)$,
allowing us to achieve larger effective sample sizes.

Second, we can often \textit{choose} $\proposal(\params)$ to be
straightforward to simulate from, such as a Gaussian distribution.
In that case, we can easily generate a series of $n$
\textbf{independently and identically distributed (iid)} samples
\begin{equation}
    \params_1, \dots, \params_n \stackrel{\iid}{\sim} \proposal(\params)
\end{equation}
These can then be used to generate an optimal estimate of
$\hat{\proposal}(\params)$ with identical weights $q_i = 1$.
Since these samples are generated \textit{randomly}, this is
referred to as a \textbf{Monte Carlo} approach for estimating
$\hat{\proposal}(\params)$ and downstream quantities.

In the case where our $n$ samples 
$\{ \params_1, \dots, \params_n \} \stackrel{\iid}{\sim} \proposal(\params)$
are indeed sampled directly from $\proposal(\params)$, our estimate
for the expectation value then reduces to
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \approx \frac{n^{-1} \sum_{i=1}^{n} f(\params_i)
    \frac{\posterior(\params_i)}{\proposal(\params_i)}}
    {n^{-1} \sum_{i=1}^{n} \frac{\posterior(\params_i)}{\proposal(\params_i)}}
\end{equation}
The corresponding weight is then
\begin{equation}
    w_i 
    \equiv \frac{\likelihood(\params_i) \prior(\params_i)}{\proposal(\params_i)}
\end{equation}
where we have again used $\likelihood(\params) \prior(\params)$ in place
of the posterior $\posterior(\params)$ since it is not known. As with the
previous case, these weights can be used to derive the evidence
\begin{align}
    \evidence 
    = \int \likelihood(\params) \prior(\params) \deriv \params
    \approx n^{-1} \sum_{i=1}^{n} \frac{\likelihood(\params_i) 
    \prior(\params_i)}{\proposal(\params_i)} = n^{-1} \sum_{i=1}^{n} w_i
\end{align}

We can interpret these weights as ways to correct for how
``far off'' our original
guess $\proposal(\params)$ is from the truth $\posterior(\params)$.
If the posterior density is higher at position
$\params_i$ relative to the proposal density, 
then we were less likely to generate
a sample at that position relative to if had simulated it directly from
the posterior and we should increase its corresponding weight.
If the posterior density is lower relative to the proposal density, 
then the alternative is true and we want to lower the weight of the
corresponding sample.

Taken together, this approach is broadly known as 
\textbf{importance sampling}, which allows us to
approximate $\hat{\posterior}(\params)$ using the following steps:
\begin{enumerate}
    \item Select a \textbf{proposal distribution} $\proposal(\params)$
    that is easy to simulate from and hopefully a good approximation of
    $\posterior(\params)$.
    \item Generate $n$ iid samples $\{ \params_1, \dots, \params_n \}$
    from $\proposal(\params)$.
    \item Compute the corresponding \textbf{importance weight}
    $w_i = \likelihood(\params_i) \prior(\params_i) / \proposal(\params_i)$
    for each sample.
\end{enumerate}

Importance sampling serves as a useful first step for understanding how
the weights are related to different Monte Carlo sampling strategies.
For instance, if we generate samples uniformly within some $d$-dimensional 
volume such that $\proposal(\params) = 1/V$ is constant, our weights will just be
proportional to the posterior:
\begin{equation}
    w_i^{\rm unif} 
    = V \likelihood(\params_i) \prior(\params_i) 
    \propto \posterior(\params_i)
\end{equation}
Alternately, if we instead take our proposal
$\proposal(\params) = \prior(\params)$ to be our prior,
we instead find our weights will be equal to the likelihood $\likelihood(\params)$:
\begin{equation}
    w_i^{\rm prior} 
    = \frac{\likelihood(\params_i) \prior(\params_i)}{\prior(\params_i)}
    = \likelihood(\params_i)
\end{equation}
Finally, if we assume $\proposal(\params) = \posterior(\params)$
is an exact approximation of the posterior, our weights will just be
constant:
\begin{equation}
    w_i^{\rm post} 
    = \frac{\likelihood(\params_i) \prior(\params_i)}{\posterior(\params_i)}
    = \evidence \frac{\posterior(\params_i)}{\posterior(\params_i)}
    = \evidence
\end{equation}
As expected, this final result guarantees a maximum
effective sample size of $n_{\rm eff} = n$.

\subsection{Relationship to Markov Chain Monte Carlo}

Now that we see how the weights relate to various Monte Carlo sampling strategies
(e.g., generating samples from the prior), we now are in a place to outline
the idea behind \textbf{Markov Chain Monte Carlo (MCMC)}. In brief,
MCMC tries generate samples in such a way that the weights
$w_1 = \dots = w_n = C$ are constant. Based on the example above, this
means MCMC seeks to generate samples proportional to
the posterior $\posterior(\params)$.
It accomplishes this by creating a \textbf{chain} of 
(correlated) parameter values $\{ \params_1 \rightarrow \dots \rightarrow \params_n \}$
over $n$ iterations such that the total amount of iterations spent in any particular
region $\delta_{\params_i}$ centered on $\params_i$ with some small volume
is proportional to the posterior density $\posterior(\params)$ contained within that region.

In other words, the ``density'' of samples generated from MCMC
\begin{equation}
    \rho(\params) \equiv \frac{n(\params)}{n}
\end{equation}
at position $\params$ integrated over $\delta_{\params_i}$ is approximately
\begin{equation}
    \int_{\delta_{\params_i}} \posterior(\params) \deriv \params
    \approx \int_{\delta_{\params_i}} \rho(\params) \deriv \params 
    \approx n^{-1} \sum_{j=1}^{n} \mathds{1}(\params_j \in \delta_{\params_i})
\end{equation}
where $\mathds{1}(\cdot)$ is the \textbf{indicator function} which is
just $1$ if the inside condition is true and $0$ otherwise. So
we just count up the number of samples within $\delta_{\params_i}$
and normalize by the total number of samples.

While this will just be approximately true for any finite $n$, as
as the number of samples $n \rightarrow \infty$ we get that
$\rho(\params) \rightarrow \posterior(\params)$ everywhere.
In theory then, once we have a reasonable enough
approximation for $\rho(\params)$, we can also get an estimate
for the evidence via:
\begin{align}
    \evidence
    = \int \frac{\likelihood(\params) \prior(\params)}{\posterior(\params)}
    \posterior(\params) \deriv \params
    \approx \int \frac{\likelihood(\params) \prior(\params)}{\rho(\params)}
    \rho(\params) \deriv \params
    = n^{-1} \sum_{i=1}^{n} 
    \frac{\likelihood(\params_i) \prior(\params_i)}{\rho(\params_i)}
\end{align}
This is just the average of the ratio 
between $\likelihood(\params) \prior(\params)$ and $\rho(\params)$
over all $n$ samples.

While this procedure gives ``ideal'' weights by simulating ``directly''
from the posterior, it is not without its drawbacks.
In particular, because the samples are correlated, the effective sample
size
\begin{equation}
    n_{\rm eff} \equiv \frac{n}{1 + \tau}
\end{equation}
where $\tau$ is the integrated \textbf{autocorrelation time}
between samples. If $\tau=0$ (i.e. $\params_i$ and $\params_{i+1}$ are
uncorrelated), then every sample is independent
and $n_{\rm eff} = n$. Conversely, if $\tau = n - 1$
(i.e. $\params_1 = \dots = \params{n}$) then every sample is
100\% correlated and $n_{\rm eff} = 1$. A driving concern
of MCMC methods is generating samples in such a way that
$\tau$ is small and $n_{\rm eff}$ is as close to $n$ as possible.

To summarize, the idea behind MCMC is to simulate a series of
values in a way that their density after a given amount
of time follows the underlying posterior. Then, 
we can estimate the posterior at any particular location by simply
counting up how many samples we simulate there and normalizing by
the total number of samples we generated. This procedure is incredibly
intuitive and part of the reason MCMC methods have 
become so widely adopted. We will return to ways to generate these
samples later.

\subsection{``Approximating the Posterior'' with Samples}

\textbf{START HERE. 
Why are we doing MCMC? 
Because in general we can get better approximations than the grid.
And therefore need fewer samples overall. More efficient.
But this doesn't mean we actually are able to 
``approximate the posterior''; if we could do that, we'd be able to
compute the evidence. We can show via some very simple scaling arguments
with $\rho(\params)$ that this still has the curse of dimensionality.}

So far we've been talking about ``approximating the posterior'' using
samples obtained from Monte Carlo methods. But what exactly does that mean?
While it's clear that as $n \rightarrow \infty$ that
$\hat{\posterior}(\params) \rightarrow \posterior(\params)$, how many
samples do we need to really be in that limit?

To get a rough idea, let's start with the assumption
that we need a minimum of
two samples to characterize the posterior in each dimension
(one sample just gives us a single point).
As an example, let's imagine that we hope to approximate
the posterior by expanding around the \textit{maximum-a-posteriori}
estimate $\params_{\rm MAP}$ (i.e. where the posterior $\posterior(\params)$
is maximized) by assigning a sample to the left and right of $\params_{\rm MAP}$
in each dimension. This minimal procedure requires $2^d$ samples:
2 in 1-D for each side, 4 in 2-D for each
quadrant, 8 in 3-D for each orthant, etc.
This quickly leads to an insane number of samples 
required as the dimensionality becomes large. For instance,
allocating a sample to each \textbf{orthant} in 30
dimensions requires $2^{30} \sim 10^{9}$ samples.

While the above argument is straightforward, there are 
some possible objections. Most immediately, we can
provide a direct ``counterexample'' to the argument above using
$d$-dimensional Gaussian distribution $\Normal{\meanvec}{\cov}$
with mean $\meanvec$ and covariance $\cov$. It is well known
that we only need on order $d$ samples to estimate the mean and $d^2$
to estimate the covariance. Characterizing the
distribution with Monte Carlo methods (e.g., MCMC) then only
should require $n \sim d^2 \ll 2^d$ samples.

Unfortunately, this reasoning ignores a huge caveat:
\textit{the assumption that the posterior is Gaussian}.
In general, however, how are you supposed to know
this without checking how the distribution behaves everywhere?
Showing that this assumption is valid then
requires exploring the entire distribution in every dimension
to make sure things don't deviate from what you'd expect.
And since the number of orthants goes as $2^d$, this
means we need a minimum of $2^d$ samples.

We can formally summarize this as:
\begin{equation}
    \hat{\posterior}(\params) \approx \posterior(\params)
    \quad\quad {\rm for} \quad n \gtrsim k^d
\end{equation}
In other words, the number of samples required
to effectively ``approximate'' the posterior increases 
exponentially with dimensionality $d$, where the scaling
$k\geq 2$ depends on the precision of the approximation needed.

This seems disappointing: why use Monte Carlo methods
at all if its ability to approximate the posterior
scales so poorly with dimensionality? Well, that's because
\textit{most of the time we don't actually care about
approximating the entire posterior}. Instead, we are
often interested in the expectation of functions
$f(\params)$ conditioned on the data, which only requires
\textit{integrating} over the posterior:
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    = \int f(\params) \posterior(\params) \deriv \params
\end{equation}

Fortunately, computing these approximations to reasonably
high precision often doesn't require that we have approximated the
posterior to high precision everywhere, but rather only in the
places that really matter. This enables us to use
methods such as MCMC to approximate these expectations as
\begin{equation}
    \meanwrt{f(\params)}{\posterior} 
    \approx \int f(\params) \rho(\params) \deriv \params
    \approx n^{-1} \sum_{i=1}^{n} f(\params_i)
\end{equation}
using the chain of MCMC parameter states
$\{ \params_1 \rightarrow \dots \rightarrow \params_n \}$.
This logic also applies to lower-dimensional (e.g., 1-D or 2-D)
marginal distributions, which marginalize over the sparse
sampling in all other dimensions to generate an accurate
lower-dimensional representation of the posterior.

\section{Where is the posterior?}

Fundamentally, computing any expectation
over the posterior $\meanwrt{f(\params)}{\posterior}$ requires
integrating over the entire domain
of our parameters $\params$. Understanding how the volume
of this domain behaves (i.e. how many parameter combinations
there are) is therefore key to understanding
why Monte Carlo approximations scale so poorly as a function
of dimensionality.

\subsection{Volume}

To start, let's consider the
\textbf{$d$-cube} with side length $\ell$ in all dimensions.
It's volume scales as
\begin{equation}
    V(\ell) = \prod_{i=1}^{d} \ell = \ell^d
\end{equation}
The differential volume element between $\ell$ and
$\ell + \deriv \ell$ is
\begin{equation}
    \deriv V(\ell) = d\ell^{d-1}\deriv\ell \propto \ell^{d-1}\deriv\ell
\end{equation}

This exponential scaling with dimensionality means that volume becomes
increasingly concentrated in thin shells located in regions located
progressively further away from the center of the $d$-cube.
As an example, consider the length-scale
\begin{equation}
    \ell_{50}/\ell = 2^{-1/d}
\end{equation}
that divides the cube into two equal-sized regions
with 50\% of the volume contained interior to $\ell_{50}$ and
50\% of the volume exterior to $\ell_{50}$. 
In 1-D, this gives $\ell_{50}/\ell = 0.5$ as we'd
expect. In 2-D, this gives $\ell_{50}/\ell \approx 0.7$. In 3-D,
$\ell_{50}/\ell \approx 0.8$. In 7-D, $\ell_{50}/\ell \approx 0.9$.
By the time we get to 15-D, we have $\ell_{50} /\ell\approx 0.95$
so that 50\% of the volume is located in the last 5\% of the 
length-scale near the boundary of the unit cube prior.

While the constants change, in general this argument holds for
any shape in high dimensions.
% Another useful example to
% consider is the \textbf{$d$-sphere}, which has a volume of
% \begin{equation}
%     V(r) = \frac{\pi^{d/2}}{\Gamma(d/2 + 1)} r^d \propto r^d
% \end{equation}
% and a differential volume element of
% \begin{equation}
%     \deriv V(r) = \frac{d\pi^{d/2}}{\Gamma(d/2 + 1)} r^{d-1} \deriv r 
%     \propto r^{d-1} \deriv r
% \end{equation}
% Since the $d$-sphere follows the same scaling as the $d$-cube, 
% it also exhibits the same behavior as the case described above with
% progressively more volume located in regions away from the center
% as the dimensionality increases.

\subsection{Mass}

We now turn our attention to the posterior $\posterior(\params)$.
Since we are almost always interested in computing
expectations over the posterior, we want to know
where the integrand $\posterior(\params) \deriv \params$ in
\begin{equation}
    1 = \int \posterior(\params) \deriv \params
\end{equation}
is maximized. Since $\posterior(\params)$ is the
posterior density and $\deriv \params$ is a differential
volume element, we can interpret this combined
$\posterior(\params) \deriv \params$ term as the
\textbf{posterior mass}. We want to find out where
this mass is generally located.

To make the integrand a little easier to conceptualize,
let's imagine that $\params = (x, y, z)$ 
and $\posterior(x,y,z)$ is
spherically symmetric. While we could imagine trying to
integrate over $\posterior(x,y,z)$ directly in terms of
$\deriv x \deriv y \deriv z$, it is almost always
easier to instead integrate over such a distribution
in ``shells'' with differential volume
$\deriv V(r) = 4 \pi r^2 \deriv r$
as a function of radius
$r = \sqrt{x^2 + y^2 + z^2}$. This allows us
to rewrite the integral as
\begin{equation}
    \int \posterior(x,y,z) \deriv x \deriv y \deriv z
    = \int \posterior(r) 4 \pi r^2 \deriv r
    = \int \tilde{\posterior}(r) \deriv r
\end{equation}
where $\tilde{\posterior}(r) = 4 \pi r^2 \posterior(r)$
is the posterior mass.
This result implies that the posterior mass isn't
just the region where the posterior takes on the
largest \textit{value}, but instead
is defined by the region that contains 
the largest \textit{amount} of the overall posterior.
More colloquially, this just means that a 
small handful of excellent fits to the data can
be easily overwhelmed by a substantially larger number
of mediocre fits.

Although not all posterior densities can be expected to
be spherically-symmetric, in general we can
rewrite the integral over $\params$ as a volume integral
over $V$ defined by some unknown iso-posterior 
contours\footnote{Indeed, some Monte Carlo methods such as 
Nested Sampling actually are designed to 
evaluate this type of volume integral explicitly.}
\begin{equation}
    \int \posterior(\params) \deriv \params
    = \int \posterior(V) \deriv V
\end{equation}
where again the size of each volume element
$\deriv V \sim r^{d-1} \deriv r$ roughly scales
exponentially with the number of dimensions. So the basic
intuition we get from the simple spherically-symmetric case
still applies.

In terms of the Monte Carlo methods where we want to
approximate the posterior using random samples, this
means that while the highest \textit{concentration}
of samples will be located in the regions of highest
posterior density, the largest \textit{amount} of samples
will actually be located in the regions of highest posterior
mass. Since this implies that a ``typical'' sample 
(picked at random) will most likely be located in this
region of high posterior mass,
this region is also commonly referred to
as the \textbf{typical set}.

\subsection{Gaussian Case}

As a concrete example, let's consider
the case where the posterior $\posterior(\params)$
is a $d$-D Gaussian distribution
with mean $\meanvec = 0$ and covariance $\cov = \sigma^2\mathbf{I}$,
where $\mathbf{I}$ is the identity matrix.
The posterior mass is then
\begin{align}
    \posterior(V) \deriv V(r)
    = \tilde{\posterior}(r) \deriv r
    &= \frac{2}{(2\sigma^2)^{d/2} \Gamma(d/2)}
    e^{-r^2/2\sigma^2} r^{d-1} \deriv r \\
    &\propto e^{-r^2/2\sigma^2} r^{d-1} \deriv r \nonumber
\end{align}
where $r = |\params|$ is the magnitude of the 
position.\footnote{Note that this is closely related
to the chi-square distribution.}

The \textbf{typical radius} $r_{\rm peak}$ 
where the posterior mass peaks
and a sample is most likely to be located
can be derived by setting the derivative of the above term to $0$.
Solving then gives
\begin{equation}
    r_{\rm peak} = \sqrt{d-1} \sigma
\end{equation}
In other words, while in 1-D a typical sample
is most likely to be located at the peak of the 
distribution with $r_{\rm peak} = 0$, in higher dimensions
this changes quite drastically. While $r_{\rm peak} = 1\sigma$
in 2-D, it is $2\sigma$ in 5-D, $3\sigma$ in 10-D, and $5\sigma$
in 26-D. This is a direct consequence of the
huge amount of volume at larger radii in high dimensions:
although a sample at $r=5\sigma$ away from the \textit{maximum-a-posteriori}
position at $r=0$ is a not a great model, the number of
parameter combinations available at $r=5\sigma$ is enormous.

In general, we expect the posterior mass to comprise
a \textbf{Gaussian shell} centered at some radius
\begin{equation}
    r_{\rm mean}
    = \int_0^\infty r \tilde{\posterior}(r) \deriv r
    = \sqrt{2} \frac{\Gamma\left(\frac{d+1}{2}\right)}
    {\Gamma\left(\frac{d}{2}\right)} \sigma
    \approx \sqrt{d} \sigma
\end{equation}
with a standard deviation of
\begin{equation}
    \Delta r_{\rm mean}
    = \sqrt{\int_0^\infty r^2 \tilde{\posterior}(r) \deriv r 
    - r_{\rm mean}^2}
    = \sigma \sqrt{d - 2 
    \left(\frac{\Gamma\left(\frac{d+1}{2}\right)}
    {\Gamma\left(\frac{d}{2}\right)}\right)^2}
    \approx \frac{\sigma}{\sqrt{2}}
\end{equation}
where the approximations are taken for large $d$.
This result illustrates that
\textit{the majority of the posterior mass $\tilde{\posterior}(r)$ 
is located progressively further away from the peak
posterior density $\posterior(r=0)$ as the dimensionality
increases.} This has immediate implications for 
how MCMC methods will behave.

\section{Markov Chain Monte Carlo}

Recall that the goal of MCMC is to generate samples
such that their density $\rho(\params)$ after
some amount of time follows the posterior
density $\rho(\params)$. However, as we just described,
the bulk of the posterior mass $\tilde{\posterior}(r)$
is actually concentrated in a thin shell
surrounding the \textit{maximum-a-posteriori} position
$\params_{\rm MAP}$. 
\textbf{The goal of MCMC is thus very clear:
efficiently generate samples from the bulk of
the posterior mass}.

Unfortunately, we don't actually
know where the posterior mass is located beforehand (if we did,
we wouldn't need to use Monte Carlo methods like MCMC to approximate
it). This means we will need to develop efficient algorithms
that enable our MCMC to generate a chain of states
that can ``explore'' the posterior mass over time.
